Assessment of machine learning methods for state-to-state approaches

It is well known that numerical simulations of high-speed reacting flows, in the framework of state-to-state formulations, are the most detailed but also often prohibitively computationally expensive. In this work, we start to investigate the possibilities offered by the use of machine learning methods for state-to-state approaches to alleviate such burden. In this regard, several tasks have been identified. Firstly, we assessed the potential of state-of-the-art data-driven regression models based on machine learning to predict the relaxation source terms which appear in the right-hand side of the state-to-state Euler system of equations for a one-dimensional reacting flow of a N$_2$/N binary mixture behind a plane shock wave. It is found that, by appropriately choosing the regressor and opportunely tuning its hyperparameters, it is possible to achieve accurate predictions compared to the full-scale state-to-state simulation in significantly shorter times. Secondly, we investigated different strategies to speed-up our in-house state-to-state solver by coupling it with the best-performing pre-trained machine learning algorithm. The embedding of machine learning methods into ordinary differential equations solvers may offer a speed-up of several orders of magnitude but some care should be paid for how and where such coupling is realized. Performances are found to be strongly dependent on the mutual nature of the interfaced codes. Finally, we aimed at inferring the full solution of the state-to-state Euler system of equations by means of a deep neural network completely by-passing the use of the state-to-state solver while relying only on data. Promising results suggest that deep neural networks appear to be a viable technology also for these tasks.

==> src/Algorithms.tex <==
\section{Machine Learning Algorithms}
\label{sec:MLAs}

\paragraph {Kernel Ridge Regression.} Kernel ridge regression generalizes the linear ridge regression model toward nonlinear functions. The non-linearity is incorporated by mapping the data from the input space into a different space called "feature space", aiming to transform the original, nonlinear regression task into a linear task in feature space. In general it is not obvious how to choose the mapping function $\varphi$. Often the most suitable functions are rather complex and result in infinite dimensional feature spaces. Since many learning algorithms only require dot products between the data vectors, this can be handled using the so-called kernel trick: instead of mapping the data and computing the inner product in feature space, it is possible to use a kernel function k(x,x') to do it in one operation and leave the mapping function and feature space completely implicit. 
According to Mercer's theorem any symmetric positive semi-definite function allows for an inner product representation %k(x,x′)=<φ(x),φ(x′)>.
Some commonly used kernels are listed in Table ?. Here ||x|| corresponds to a Euclidean L2-norm, while |x| corresponds to a Manhattan, or city block, L1-norm. Note that now a kernel function needs to be chosen instead of a complex mapping function. The kernel function facilitates treating nonlinear problems by mapping into infinite-dimensional feature spaces. Mathematically they allow us to move our problem from a d-dimensional input space into an n-dimensional space spanned by then data points. There we can focus on the task relevant subspace to solve our problem. Often several kernel functions yield good results for the same data set, however, the optimal choice cannot be assessed beforehand and needs to be determined in statistical tests. %In this paper both the Gaussian as well as Laplacian kernels showed promising results in preliminary experiments and will be used to train our models.
Kernel ridge regression uses a quadratic constraint on the norm of the weights $\alpha$ and solves the nonlinear regression problem
%∑∑∑λααα−+·=α==yfxkxxfxkx xmin((   ))(    ,)with   (  )(    ,)iniiijiijjinii12,1(10)
The minimization problem has the closed form solution
%α=(K+λ·I)−1y, 
where y is the training label vector and K is the kernel matrix. The regularization parameter $\lambda$ is again a hyper-parameter, as are any kernel dependent parameters, such as, in the case of the Gaussian and Laplacian kernel, the kernel width $\sigma$. They need to be chosen separately within a model selection procedure. 
One main drawback of kernel-based methods such as kernel ridge regression is that they are in general not well suited for large data sets.

\paragraph {Support Vector Regression.} Support vector regression (SVR) is a kernel-based regression method, which can be depicted as a linear regression in feature space-like kernel ridge regression. Unlike kernel ridge regression, SVR is based on an $\epsilon$-insensitive loss function (Eq. ?), where absolute deviations up to $\epsilon$ are tolerated. The corresponding convex optimization problem has a unique solution, which cannot be written in a closed form but is determined efficiently using numerical methods for quadratic programming (see~\cite{scholkopf2002learning, platt1998fast}). One key feature of SVR is sparsity, i.e. only a few of the data points contribute to the solution. These are called support vectors. Though the number of support vectors is generally small it may rise dramatically for very complex or very noisy problems. For a given data set with n data points, SVR solves the optimization problem 
%∑∑∑ααααεαααα−−*−*−+*+−*αα*===kx  xymax12()()(,)() (),ijniijj ijiniiiniii,,111ii(11)
subject to the following constraints
%∑αααα−*=≤*≤=C()0and0,iniiii1(12)
where C is a regularizing hyper-parameter. The regression function takes the form
%∑αα=−*=fxkxx()()( ,  )inii i1(13)
%Based on preliminary experiments the Gaussian and Laplacian kernel were selected for the support vector regression employed in this study.
Thus, two hyper-parameters need to be optimized, namely the kernel width $\sigma$ and the parameter C.

\paragraph{Multilayer Neural Networks.} In multilayer neural networks, the function $f$ that maps inputs to outputs is implemented by a directed set of interconnected units, which are called neurons. Each neuron implements a basic computation, typically 
%y= tanh(∑iwixi+b), 
where {xi} are the inputs to the neuron, {wi} are the weights, b is a constant, and y is the neuron output. A neuron is depicted in Figure ? (left). The neurons are placed in a layered architecture as shown in Figure ? (right). The mapping between inputs and outputs is implemented by the following computation
%:=·+≤≤==·−iLyhWhbhxVhtanh()for 1,   andtanh()iiiiL10
The matrices W1,...,WL, V and vectors b1,...,bL are the model parameters and have to be learned from data. Neural networks are generally trained one sample at a time, using stochastic gradient descent. Typically the training procedure requires a large number of iterations but scales well with the number of samples. Thus neural networks are able to absorb a large number of data points. An advantage of neural networks is that they are able to automatically extract, layer after layer, the representation necessary for solving the task. As a downside, neural networks algorithms typically have multiple local minima, i.e. if a parameter configuration where any small change to this parameter set only reduces the model quality is discovered, we have in general not reached the optimal parameter set. This implies that successful training requires an experienced choice of parametrizations, learning rates, and initialization in order to find the best parameter set.

\paragraph{k-Nearest Neighbor.} A further well-known nonlinear algorithm is the k-nearest neighbor method (KNN). For each new sample x the k nearest training samples are selected, and the predominant label among those neighbors determines the label in classification tasks; for regression tasks the (weighted) mean label value is taken into account. Despite its simplicity the KNN approach often works well, if a reasonable distance measure is applied (typically the Euclidean distance). Only one hyper-parameter k needs to be determined, e.g. by cross-validation.

==> src/Data.tex <==
\section{Data set and data representation}
\label{sec:data}
In this section we describe the data set that is used to build and validate the ML models for the relaxation terms regression. The quality and applicability of ML prediction models inherently depend on the size and diversity of the underlying data set. Moreover, the numerical representation of the included coefficients dependencies is a critical aspect for model quality~\cite{Rupp2012, Hansen2013, rupp2015machine}.

\emph{Data set.} The data set for this task was generated by an in-house Matlab code for the solution of STS one-dimensional relaxation process behind a shock wave. Detailed description and results of the code can be found in~\cite{campoli2020models}. The data set contains the molecular and atomic relaxation terms as functions of the distance from the shock, elapsed time, temperature and number densities. In the present assessment we considered the temperature to be the only independent variable, thus a single-input, multi-output regression, where the multiplicity of the prediction is given by the vibrational levels of the molecular species was performed. The data set was divided in the following way: 75\% of samples were used for training, whereas the remaining 25\% were used for testing, using the \texttt{train\_test\_split} built-in function. Hyperparameters are parameters that are not directly learned within estimators. They are passed as arguments to the constructor of the estimator classes. It is possible and recommended to search the hyperparameter space for the best cross-validation score. We used \texttt{GridSearchCV} to tune the hyperparameters. Each method was run with a preset grid of input parameters, detailed in Tab.~\ref{tab:methods}. The optimal setting of the parameters was determined based on 10-fold cross-validation performed on training data only. The setting with the best $R^2$ score across all folds was used for re-training the algorithms on the whole training data.

\emph{Data representation.} In order to apply machine learning, the information encoded in the relaxation terms needs to be converted into an appropriate vectorial form. This vector representation is very important for the success of the learning approach. Only if all relevant information (important feature) is appropriately encoded in the vector will the machine learning algorithm be able to infer the relation between inputs and outputs, correctly. Different system representations can be proposed and finding the optimal representation is the subject of ongoing research, and an in-depth discussion of all of them is beyond the scope of this work.

==> src/MLAforSTS.tex <==
\section{Machine learning coupled with CFD solver}\label{sec:coupling}

In the previous task, several MLAs have been compared to perform regression of relaxation terms and transport coefficients defined in the framework of the STS formulation. It was found that by an appropriate selection of hyper-parameters, through a cross-validation technique, satisfactorily accurate predictions can be achieved in short times. A logical continuation of the previous task, may then consist in exploiting the potential of the MLAs by directly coupling them with a CFD solver in order to relief it from the computationally expensive loops associated to the transport and kinetic part. In the present section, a coupling between the best-performing MLA, respect to the results of the previous section, and a CFD solver is explored and sketched in Fig.~\ref{fig:ML4CFD}. The datasets of reaction rate and transport coefficients which have been described in the previous sections are generated, by running an in-house developed Matlab code and the KAPPA library, respectively. These datasets feed the ML block which performs the training, test and validation and after evaluating the best-scoring algorithm which is subsequently used to generate the prediction model. On the application side, an ML interface was implemented into the SPARK code. By calling the polymorphic procedure interface it is possible to select at runtime the model to be used for the computation of the relevant quantities. When the ML method is chosen, the Kinetic and Transport module interface call the pre-trained ML model.
Calling python from Fortran is known as "embedding", but python is not designed to be an embedded language, so this may introduce a significant latency in the working cycle. There may be several ways to embed python within a Fortran code:
\begin{itemize}
    \item Fortran intrinsics. The execute\_command\_line allows to run a shell command, synchronously or asynchronously but may penalize the performance.
    \item Python's C-API. This is the most general way, but would involve writing a conspicuous amount of C wrapper code.
    \item Cython. Cython is typically used to call C from python, but it is possible to use the other way around.
    \item CFFI. This python package has a very convenient feature for embedding python.
\end{itemize}

\input{SPARK_MLA}

==> src/Methodology.tex <==
\section{Methodology}
\label{sec:methodology}

In this section we describe several methodological aspects relative to the ML workflow, such as the model assessment and selection, the data set generation and representation that are used to build and validate the ML models in the present study. 
\emph{Model assessment.} The overall goal of machine learning is to establish high-quality prediction models. The quality of a model is measured by the \textit{generalization error}, the expected prediction error on new data or extrapolation ability. As the error on new data cannot be known, one must approximate it by an inference procedure, which allows one to judge how well the learning machine generalizes. The simplest procedure separates the data set into a training and a test set. The model is then built on the training set, and the average loss over the test set (test error)

serves as an approximation of the generalization error. Averaging over the absolute error loss function results in the mean absolute error (MAE); for the squared error loss function the mean squared error (MSE) is calculated. In addition to the latter, the root mean squared error (RMSE), which estimates the standard deviation of an unbiased estimator, is also commonly reported. It is important to note that the training error does not provide an unbiased estimate of the generalization error since it decreases for models that adapt too close to the training data, i.e. overfit. To build an optimal model and assess its quality, requires large data sets, which in practice generally exceed the data available or exhaust the memory of the computational resources. Different methods ranging from a simple holdout, over \textit{k}-fold cross-validation, leave-one-out cross-validation, Monte Carlo cross-validation, up to leave-one-cluster-out cross-validation can be used for the evaluation. All these methods rely on keeping some data hidden from the model during the training process. One of the standard procedures to estimate the generalization error on limited data sets is \textit{k}-fold cross-validation. In \textit{k}-fold cross-validation the data set is randomly split into \textit{k} equally sized subsets (splits). Each of these splits serves as a test set once, while the remaining splits are used for training. In this way, \textit{k} models are built, and one prediction is generated for each available data point. The errors of the \textit{k} different models are averaged into one cross-validation error. Note that the cross-validation error is still a random variable, which depends on the initial splitting of the data into \textit{k} splits. To reduce its variance the whole process of cross-validation may be repeated several times. The number of folds \textit{k} should be chosen with respect to the number of available data points and computational capacities. Small data sets and complex tasks require larger values of \textit{k} to ensure sufficiently large training sets. In general, a \textit{k} value of 5 or 10 is usually recommended~\cite{breiman1992submodel, krstajic2014cross}.

\emph{Model selection.} To construct a learning machine, we not only need to optimize the loss function with respect to the model parameters (as done by learning algorithms), but the hyperparameters need to be chosen with care in order to regularize the optimization problem appropriately.  
Hyperparameters are parameters that are not directly learned within estimators while they are passed as arguments to the constructor of the estimator classes.
One of the standard procedures to select hyperparameters is again \textit{k}-fold cross-validation: first a number of candidate models, i.e. models with different hyperparameter settings, are specified. Then the data set assigned as the "train and model selection" set is split into \textit{k} equally sized subsets. Each candidate model is trained on (\textit{k}-1) subsets and evaluated on the remaining validation subset. As before, the training and evaluation is repeated by cycling around the validation subset. Finally, the candidate model that performed best in the majority of the \textit{k} repetitions is selected and trained on all \textit{k} subsets. 
The scikit-learn built-in function \texttt{GridSearchCV} was used to tune the hyperparameters.

\emph{Data set.} The quality and applicability of ML prediction models inherently depend on the size and diversity of the underlying data set. Moreover, the numerical representation of the included terms dependencies is a critical aspect for model quality~\cite{Rupp2012, Hansen2013, rupp2015machine}. 
The data set for this task was generated by an in-house Matlab code for the solution of STS one-dimensional relaxation process behind a shock wave. Detailed description and results of the code can be found in~\cite{campoli2020models}. The data set contains the molecular and atomic relaxation terms, $R_{ci}$, as functions of the distance from the shock, elapsed time, temperature and number densities. In the present assessment we considered the temperature to be the only independent variable, thus a single-input, multi-output regression, where the multiplicity of the prediction is given by the vibrational levels of the molecular species, was performed. The data set was divided in the following way: 75\% of samples were used for training, whereas the remaining 25\% were used for testing, using the \texttt{train\_test\_split} built-in scikit-learn function.

\emph{Data representation.} In order to apply machine learning, the information encoded in the relaxation terms needs to be converted into an appropriate vectorial form. This vector representation is very important for the success of the learning approach. Only if all relevant information (important feature) is appropriately encoded in the vector the machine learning algorithm will be able to correctly infer the relation between inputs and outputs. Different representations can be proposed and finding the optimal representation is the subject of ongoing research, and an in-depth discussion is beyond the scope of this work.

\emph{Data preprocessing.} Most machine learning methods are not invariant under scaling of the input. Typically each input dimension (feature) is standardized to have zero mean and unit variance. The standardization ensures that all inputs are penalized equally strong within regularization, which typically produces better results. Moreover, the standardization generally improves the condition of the optimization problem and
alleviates the selection of good model hyperparameters. 

A general good practice is to check whether a scaling (or no scaling) better reflects the importance and relations of the features and improves the results or distorts the internal structure and relations between input dimensions. In this study the input dimensions are related and scaling proved to be advantageous for all learning methods. Consequently, the algorithms were fed with scaled data. This also favours input data consistent across multiple algorithms for the purpose of benchmarking.

Moreover, data leakage is another issue of MLAs, that is when information from outside the training data set is used to create the model. This additional information can allow the model to learn or know something that it otherwise would not know and in turn invalidate the estimated performance of the model being constructed. Such issue was avoided by using \texttt{fit\_transform} on the train data to learn and train the scaling parameters on the train data while only using \texttt{transform} on the test data with the scaling parameters learned on the train data.
A preliminary assessment of the influence of model stability and performance on data scaling was conducted. Comparable results were found by using standardized (\texttt{StandardScaler}) and normalized (\texttt{MinMaxScaler}) approaches while unscaled data introduced severe issues in the algorithmic convergence. Nevertheless, the choice of the optimal preprocessing method for the particular regressor is out of scope of this paper.

\emph{Algorithm initialization.} Different algorithm initialization may be considered, for example by randomly seeding or randomly data splitting. Both approaches have disadvantages: the results will either be biased by the choice of the random seed or by using different splits for different methods (even if by taking a median of the scores they could become independent of the initial split of the data). We initialized each of the methods with the same random seed, in order to favour results' reproducibility. 

\emph{Runtime comparison.} Training and prediction times of
most MLAs depend on the size of the training data set. Runtime obviously depends on the machine as well as the implementation used. For this reason, the numbers given here are only meant to provide generic relative guidance.
